The role of planarity in connectivity problems parameterized by treewidth

For some years it was believed that for "connectivity" problems such as Hamiltonian Cycle, algorithms running in time 2^{O(tw)}n^{O(1)} -called single-exponential- existed only on planar and other sparse graph classes, where tw stands for the treewidth of the n-vertex input graph. This was recently disproved by Cygan et al. [FOCS 2011], Bodlaender et al. [ICALP 2013], and Fomin et al. [SODA 2014], who provided single-exponential algorithms on general graphs for essentially all connectivity problems that were known to be solvable in single-exponential time on sparse graphs. In this article we further investigate the role of planarity in connectivity problems parameterized by treewidth, and convey that several problems can indeed be distinguished according to their behavior on planar graphs. Known results from the literature imply that there exist problems, like Cycle Packing, that cannot be solved in time 2^{o(tw logtw)}n^{O(1)} on general graphs but that can be solved in time 2^{O(tw)}n^{O(1)} when restricted to planar graphs. Our main contribution is to show that there exist problems that can be solved in time 2^{O(tw logtw)}n^{O(1)} on general graphs but that cannot be solved in time 2^{o(tw logtw)}n^{O(1)} even when restricted to planar graphs. Furthermore, we prove that Planar Cycle Packing and Planar Disjoint Paths cannot be solved in time 2^{o(tw)}n^{O(1)}. The mentioned negative results hold unless the ETH fails. We feel that our results constitute a first step in a subject that can be further exploited.

==> otwlogtw.tex <==
Using ideas similar to those in the reduction for {\textsc{Monochromatic Disjoint Paths}} in Theorem \ref{th:lbmdp}, we can prove that other planar problems cannot be solved in time $2^{o(\tw \log \tw)}$ unless the ETH fails.
Intuitively, we can prove lower bounds along the same ideas for problems where some information can be carried by paths that belong to the solution.
For example, this is the case of  {\sc Planar Subgraph Isomorphism}.

\probls
{\textsc{Planar Subgraph Isomorphism}}
{Two planar graphs $G$ and $H$.}
{Does $G$ contain a subgraph isomorphic to $H$?}
{The treewidth $\tw$ of $(G)$.}

\begin{theorem}\label{thm:PlanarSubgraphIso}
\textsc{Planar Subgraph Isomorphism} cannot be solved in time $2^{o(\tw \log \tw)}\cdot n^{O(1)}$ unless the ETH fails.
\end{theorem}

\input{otwlogtwgadget}

\begin{proof}
We reduce again from \textsc{$k \times k$-Hitting Set}.
Let $k \geq 3$ be an integer and $S_1, S_2, \dots, S_m \subseteq [k]\times[k]$ such that each set contains at most one element from each row of $[k]\times[k]$.
We proceed to construct a graph $G$ similar to the one for \textsc{Monochromatic Disjoint Paths}, and we simultaneously construct the graph $H$. In this section, each connected component of $H$ is called  a \emph{request}, so $H$ will consist of the union of all the constructed requests.
We now explain how we modify the expel, the color-selection, and the set gadgets.
%, and the avoid path gadget. 

 As in \textsc{Monochromatic Disjoint Paths}, we create a gadget for each row $\{r\} \times [k]$ and
make  for each of these gadgets a request $Req_r$, depicted in Fig. \ref{fig:RSI}, that chooses a path and simulates a color for each row. We will again add an appropriate set gadget ensuring that $S\cap S_i \not = \es$ for each $i \in [m]$.
For each $r \in [k]$, the request $Req_r$  simulates the path from $s_r$ to $t_r$ that appears in \textsc{Monochromatic Disjoint Paths}. The way it is inserted in the color-selection gadget simulates the color of the path $s_r \dots t_r$ and determines the paths it can use in the set gadgets, similarly to the reduction for {\sc Monochromatic Disjoint Paths}.

More precisely, we define $k+1$  graphs that do not appear anywhere else in the graph as a subgraph. For instance, we can take a grid of size $k+2$ in which we remove a different vertex every time. Let $Gr_1, Gr_2, \dots, Gr_k$ and $Gr_g$ be these grids.
Each such modified grid $Gr_i$, $i \in [k]$,  identifies the subgraph corresponding to the row $i$, while $Gr_g$ identifies the expel gadget requests.
We redefine the \emph{expel} gadget as depicted in Fig. \ref{fig:EESI} and the \emph{color-selection} gadget as depicted in Fig. \ref{fig:CSSI}. We also redefine the \emph{set} gadget as depicted in Fig. \ref{fig:SSI}, similarly to \textsc{Monochromatic Disjoint Paths} but with the new expel gadget and
a way to simulate in {\sc Planar Subgraph Isomorphism} the color we had in {\sc Monochromatic Disjoint Paths}.

The final graph we construct has the same shape depicted in Fig. \ref{fig:FG}
but with the new gadgets instead.
We define the planar graph $H$ to be the union of the $m\cdot (k-1)$ expel gadget requests  shown in Fig. \ref{fig:EESI} and the request $Req_r$ for each $r \in [k]$.

All we have to specify is that we can use the path in the set gadget that simulates the colored path in the reduction of {\sc Planar Monochromatic Disjoint Paths}  only if we choose the corresponding color in the color-selection gadget. This property is given by the fact that we look for a path where the constructed grids are spaced by the same number of vertices each time, and therefore the color selected in the color-selection gadget is preserved in each set gadget.

If $S$ is a solution of \textsc{$k \times k$-Hitting Set}, by finding the request $Req_i$ that simulates the corresponding color we can construct solution to {\textsc{Planar Subgraph Isomorphism}}, similarly to the way we found a solution of \textsc{Monochromatic Disjoint Paths}.
Conversely, for the same reason in the proof for \textsc{Monochromatic Disjoint Paths}, a solution of {\textsc{Planar Subgraph Isomorphism}} also defines a solution $S$ of \textsc{$k \times k$-Hitting Set}.
\end{proof}

